Mosaic: Efficient CPU--GPU Coordinated Block-Sparse Attention for Long-Context Decoding

Long-context LLM serving increasingly relies on CPU-resident context KV cache, driven by KV offloading and disaggregated prefill--decode execution. Although block-sparse attention reduces KV access, existing designs remain inefficient: GPU-centralized execution fetches selected KV blocks from CPU memory at each decoding step, making it PCIe-bound, while CPU--GPU partitioned execution places CPU-side sparse attention on the critical path, leaving substantial GPU time idle. This paper presents Mosaic, a CPU--GPU coordinated block-sparse attention system for efficient long-context decoding with CPU-resident context KV. Mosaic builds on three key insights: output-contribution-aware KV budgeting, head-specific and granularity-aware sparse configuration, and cross-device coordinated scheduling for sparse tasks over CPU-resident KV. Guided by these insights, Mosaic integrates a lightweight head-property predictor, a granularity--budget selector, and a priority-based scheduler to automatically configure and coordinate sparse attention, preserving output quality while improving efficiency on heterogeneous architectures. Across 2 models, 3 benchmarks, and 40 tasks, Mosaic preserves near-FULL quality while achieving a better overall quality--efficiency tradeoff than the evaluated baselines. Compared with the best-quality fixed Quest configuration, Mosaic improves TPOT by up to 3.7$\times$. We further validate Mosaic across four hardware configurations and in a large-model multi-GPU deployment.

==> 0_extended_abstract.tex <==
\title{Mosaic: Efficient CPU--GPU Coordinated Block-Sparse Attention for Long-Context Decoding}

\author{Anonymous Authors}

\maketitle

\noindent\textbf{Motivation.}
Long-context inference is becoming an increasingly important workload in LLM serving, driven by applications such as long-document understanding, multi-hop reasoning, and repository-scale code analysis~\cite{liu2025comprehensive,jiang2024minference,lai2025flexprefill,xiao2024infllm}. As context length grows, the KV cache generated during prefill can quickly exceed GPU memory capacity. This makes CPU offloading and hierarchical KV-cache management increasingly common in practical systems~\cite{chen2024magicpig,lee2024infinigen,zhang2025pqcache}. A similar deployment pattern also appears in disaggregated prefill--decode architectures, where prefill workers transfer generated KV caches to the host memory of decode workers for subsequent decoding~\cite{qin2025mooncake,liu2025lmcache}. As a result, long-context decoding often needs to access a large CPU-resident KV cache through the relatively slow CPU--GPU interconnect.

This is a systems problem because the decoding bottleneck is no longer only the attention algorithm, but also how sparse attention interacts with heterogeneous CPU--GPU execution, PCIe traffic, host-memory bandwidth, GPU utilization, and per-token latency. Block-sparse attention is a natural way to reduce the cost of accessing CPU-resident KV: it selects only a small set of query-relevant KV blocks and computes attention over them. However, sparsity alone does not guarantee end-to-end efficiency. A sparse method that preserves model quality may still leave the GPU waiting for CPU-side selection or sparse computation, while an aggressive sparse method may reduce latency only by losing too much context. The key challenge is therefore to make sparse attention both quality-preserving and system-efficient under CPU--GPU execution.

\noindent\textbf{Limitations of current approaches.}
Existing systems for long-context decoding with CPU-resident KV mainly follow two execution designs. GPU-centralized designs perform sparse selection and attention on the GPU, but still need to fetch selected KV blocks from CPU memory at every decoding step~\cite{chen2024magicpig,pan2025instattention,gao2024cost,zhang2025pqcache,lee2024infinigen}. This makes performance constrained by CPU--GPU interconnect bandwidth and can introduce extra GPU-memory overhead for sparse metadata. CPU--GPU partitioned designs instead keep only a small default KV subset on the GPU, perform sparse attention over CPU-resident KV on the CPU, and return only the attention outputs to the GPU~\cite{deng2025hgca,liuretrievalattention,chen2025ktransformers}. This reduces selected-KV transfer and avoids GPU metadata overhead, but places CPU-side top-$k$ selection and sparse attention on the decoding critical path.

Our analysis shows that CPU--GPU partitioned execution is a better starting point than GPU-centralized execution, but it is still far from optimal. It leaves substantial GPU time idle, and the idle fraction increases with context length and batch size. The bottleneck is the CPU-side sparse branch, which includes top-$k$ block selection and sparse attention over CPU-resident KV. Existing sparse-attention methods also commonly rely on fixed sparse configurations, such as a fixed block size or a fixed KV budget~\cite{tang2024quest,xiao2023streamingllm,chen2024magicpig}. These fixed settings are insufficient because attention heads differ in their retrieval behavior, output importance, and sensitivity to retrieval granularity. Thus, the problem is not simply to choose a smaller KV budget; the system must decide where sparse attention is needed, how much KV each head should retrieve, at what granularity, and how to schedule the remaining sparse work across CPU and GPU.

\noindent\textbf{Key ideas.}
This paper presents Mosaic, a CPU--GPU coordinated block-sparse attention system for efficient long-context decoding with CPU-resident context KV. Mosaic is built on three ideas. First, KV budget allocation should be output-contribution-aware rather than score-based. Attention scores alone do not necessarily reflect how much a head contributes to the final attention output. A head can receive high attention mass while contributing little to the output magnitude, and over-budgeting such heads wastes CPU-side sparse computation. Mosaic therefore allocates KV budget by considering both attention-output deviation and each head's relative contribution, reducing unnecessary budget for low-impact heads while preserving output quality.

Second, sparse configuration should be both head-specific and granularity-aware. Not every head needs CPU-side retrieval. Some heads behave like streaming heads and can be handled by the default GPU-resident KV subset, avoiding CPU-side top-$k$ selection and sparse attention entirely. For heads that do require retrieval, block size and KV budget are predictably coupled: a coarser granularity may need a different budget to preserve quality, while a finer granularity may increase selection overhead. Mosaic therefore uses a lightweight head-property predictor to classify heads and predict the budget--granularity relationship, then uses a granularity--budget selector to choose the sparse configuration for each retrieval head or GQA group.

Third, efficient sparse attention over CPU-resident KV requires coordinated CPU--GPU scheduling rather than static placement. For sparse attention, PCIe transfer can largely offset the GPU's compute advantage, making the end-to-end latency gap between CPU and GPU narrower than expected. Meanwhile, CPU-side sparse execution has high variance because selected KV sizes differ across heads and decoding steps. Mosaic uses a priority-based scheduler that places sparse attention tasks into a shared queue and dynamically dispatches them to CPU and GPU workers according to task priority and runtime availability. This coordinated scheduling reduces attention completion time and improves GPU utilization without requiring precise cost prediction for every task.

\noindent\textbf{Overview of results.}
We evaluate Mosaic on an AMD EPYC 7V13 server with 24 CPU cores, 220 GB host memory, and an NVIDIA A100 80 GB GPU connected through PCIe 4.0. We use two instruction-tuned long-context models, Llama-3.1-8B-Instruct and Qwen2.5-7B-Instruct, both supporting up to 128K context length and using GQA~\cite{grattafiori2024llama,yang2024qwen2}. We evaluate generation quality on L-Eval, LongBench, and RULER, covering 40 tasks across realistic open-ended generation, multilingual long-context tasks, code, and controlled synthetic long-context workloads~\cite{an-etal-2024-l,bai2024longbench,li-etal-2025-ruler}. We compare against FULL attention, Quest under multiple fixed block-size and budget settings, StreamingLLM, and MagicPIG~\cite{tang2024quest,xiao2023streamingllm,chen2024magicpig}. We report generation quality using the benchmark-specific metrics and decoding efficiency using time per output token (TPOT).

Mosaic preserves generation quality close to FULL attention. On L-Eval, Mosaic trails FULL attention by only 0.24 on Qwen2.5-7B-Instruct and 0.26 on Llama-3.1-8B-Instruct. On LongBench, the gap is even smaller: Mosaic is 0.13 below FULL on Qwen and slightly exceeds FULL by 0.02 on Llama. On RULER, Mosaic achieves 72.53 accuracy on Qwen and 85.03 on Llama, only 1.54 and 0.78 below FULL, respectively. Across LongBench and L-Eval, Mosaic reaches 99.6% of FULL-attention average quality, outperforming StreamingLLM and MagicPIG and matching or approaching the best fixed Quest configuration.

Mosaic also improves decoding efficiency while preserving this quality. Compared with Quest($16$, $0.05$), the fixed Quest configuration with the best quality, Mosaic improves TPOT by 1.7$\times$--3.0$\times$ on Qwen and 2.1$\times$--3.2$\times$ on Llama. The gain grows with batch size and context length; for example, at batch size 4 on Qwen, speedup increases from 1.7$\times$ at 32K context to 2.8$\times$ at 128K context. Under mixed-length workloads, Mosaic also consistently outperforms Quest($16$, $0.05$); on Llama, the median TPOT speedup increases from about 2.3$\times$ when lengths are sampled from 16K--64K to about 2.6$\times$ when lengths are sampled from 32K--128K. These results show that Mosaic is especially useful when attention becomes a larger fraction of decoding time.

Finally, ablation studies confirm that Mosaic's gains come from all three design choices. Output-contribution-aware budgeting gives a better accuracy--latency tradeoff than score-based budgeting. Dynamic granularity--budget selection reduces TPOT with almost no quality loss compared with fixed granularity, and streaming-head skipping further removes unnecessary CPU-side work. Priority-based scheduling outperforms no parallelism, uniform allocation, and length-based allocation under mixed-length workloads. Mosaic also substantially reduces GPU idle time: under a representative Qwen setting with batch size 4 and 32K context, the GPU idle ratio drops from 70.65% with Quest($16$, $0.05$) to 45.78% with Mosaic. The predictor overhead remains small, ranging from 1.9% to 8.2% of total execution time and decreasing as batch size or context length increases.

Overall, Mosaic advances the state of the art by showing that long-context sparse attention over CPU-resident KV should be optimized as a heterogeneous systems problem. By jointly optimizing output-aware budget allocation, head-specific sparse configuration, and CPU--GPU coordinated scheduling, Mosaic turns block-sparse attention into robust end-to-end performance gains while preserving near-FULL generation quality.

